Prompting AI Art: An Investigation into the Creative Skill of Prompt Engineering

We are witnessing a novel era of creativity where anyone can create digital content via prompt-based learning (known as prompt engineering). This paper investigates prompt engineering as a novel creative skill for creating AI art with text-to-image generation. In three consecutive studies, we explore whether crowdsourced participants can 1) discern prompt quality, 2) write prompts, and 3) refine prompts. We find that participants could evaluate prompt quality and crafted descriptive prompts, but they lacked style-specific vocabulary necessary for effective prompting. This is in line with our hypothesis that prompt engineering is a new type of skill that is non-intuitive and must first be acquired (e.g., through means of practice and learning) before it can be used. Our studies deepen our understanding of prompt engineering and chart future research directions. We conclude by envisioning four potential futures for prompt engineering.

==> FIG/FIG-BOXPLOTS.tex <==
%TC:ignore
\noindent%
\begin{figure}[htb]%
\centering%
\begin{tabular}{cc}%
  \includegraphics[width=.48\linewidth]{figures/boxplots/study2-boxplots-img.pdf}
% \vspace{10pt}
% \\
&
  \includegraphics[width=.48\linewidth]{figures/boxplots/study2-boxplots-prompt.pdf}
\\
    a) Image ratings
&
    b) Prompt ratings
\\
\end{tabular}
\caption{Absolute Category Rating (ACR) scores by workers ($N=XXX$) for images (a) and prompts (b) with high aesthetic quality (H1--H10) and low aesthetic quality (L1--L10) in Study 2.}
\Description{A woman and a girl in white dresses sit in an open car.}
\label{fig:study2:boxplots}
\end{figure}
%TC:endignore


==> FIG/FIG-CORRELATION.tex <==
%TC:ignore
\begin{figure}[htb]
\centering
\begin{tabular}{c}
  \includegraphics[width=.9\linewidth]{figures/correlations-H.pdf}
\\
    a) High quality prompts (x-axis) and images (y-axis)
\vspace{10pt}
\\
  \includegraphics[width=.9\linewidth]{figures/correlations-L.pdf}
\\
    b) Low quality prompts (x-axis) and images (y-axis)
\\
\end{tabular}
\caption{Spearman correlations between aesthetic appeal ratings by workers ($N=X$) in Study 2.}
\Description{A woman and a girl in white dresses sit in an open car.}
\label{fig:study2:graphs}
\end{figure}
%TC:endignore


==> FIG/FIG-SCATTERPLOT.tex <==

%TC:ignore
\begin{figure}[htb]%
\centering%
\includegraphics[width=.9\linewidth]{figures/scatterplots/guesses.pdf}%
\caption{\hl{Scatterplot showing a two-tailed distribution of the relative number of correct responses per worker ($N=128$).
Some workers correctly identified the style in 100\% of their completed tasks, but none of the artists (top left) and vice versa (bottom right).
Many workers were not able to neither identify the artist name nor artwork style in any of their tasks (bottom left).
However, about 30\% of the workers correctly identified both the artist and style in all of their tasks (top right).}}%
\label{fig:scatterplot}
\end{figure}%
%TC:endignore



==> FIG/FIG-STUDY2-EXP.tex <==
%TC:ignore
\noindent%
\begin{figure}[htb]%
\centering%
\begin{tabular}{cc}%
  \includegraphics[width=.65\linewidth]{figures/study2/study-2-error.pdf}
% \vspace{10pt}
% \\
\end{tabular}
\caption{As art experience increases, the average error in differences between the textual Prompt and visual Artwork decreases.
The x-axis represents the sum of the responses to two 5-point Likert-scale questions about self-rated familiarity with art and recent visits to art shows or museums.
}
\Description{}
\label{fig:study2:error}
\end{figure}
%TC:endignore


==> FIG/FIG-WORDCLOUDS.tex <==
%
%TC:ignore
\begin{figure}[htb]%
\centering%
% \raggedright
\begin{subfigure}[b]{0.3\textwidth}%
    \includegraphics[width=\linewidth]{figures/wordclouds/study3-wordcloud-NN.pdf}
    \subcaption{%
        \centering
        % Nouns
        \texttt{NN}
        % {\small $M=3.27$,~$SD=3.36$}
    } % (\texttt{NN})
    \label{fig:study2:graphs:a}
\end{subfigure}
\begin{subfigure}[b]{0.205\textwidth}
    \includegraphics[width=\linewidth]{figures/wordclouds/study3-wordcloud-JJ.pdf}
    \subcaption{
        \centering
        % Adjectives
        \texttt{JJ}        
        % \\
        % {\small $M=1.65$,~$SD=1.95$}
    } % (\texttt{JJ})
    \label{fig:study2:graphs:b}
\end{subfigure}
\begin{subfigure}[b]{0.205\textwidth}
    \includegraphics[width=\linewidth]{figures/wordclouds/study3-wordcloud-VB.pdf}
    \subcaption{
        \centering
        % Verbs
        \texttt{VB}        
        % {\small $M=0.36$,~$SD=1.02$}
    } % (\texttt{VB})
    \label{fig:study2:graphs:c}
\end{subfigure}
\begin{subfigure}[b]{0.127\textwidth}
    \includegraphics[width=\linewidth]{figures/wordclouds/study3-wordcloud-IN.pdf}
    \subcaption{
        \centering
        % Prepositions
        \texttt{IN}
        % {\small $M=1.78$,~$SD=2.27$}
    } % (\texttt{IN})
    \label{fig:study2:graphs:d}
\end{subfigure}
\begin{subfigure}[b]{0.091\textwidth}
    \includegraphics[width=\linewidth]{figures/wordclouds/study3-wordcloud-CD.pdf}
    \subcaption{
        \centering
        % Cardinals
        \texttt{CD}
        % \\
        % {\small $M=0.07$,~$SD=0.29$}
    } % 
    \label{fig:study2:graphs:e}
\end{subfigure}
\caption{Wordclouds created from the 375 prompts provided by 125 workers in Study 3, split into nouns (\texttt{NN}), adjectives (\texttt{JJ}), verbs (\texttt{VB}), prepositions (\texttt{IN}), and cardinal numbers (\texttt{CD}). English stop words have been removed in this figure.
}
\Description{Wordclouds of tokens from 375 crowdsourced prompts.}%
\label{fig:study34:wordclouds}%
\end{figure}%
%TC:endignore
%

==> TAB/TABLE-HIGH-BAK.tex <==

%TC:ignore
\noindent%
\begin{tabularx}{\textwidth}{%
    >{\hsize=.33\hsize}X
    >{\hsize=.33\hsize}X
    >{\hsize=.33\hsize}X
}%
    % H1
      \vspace{0pt} \includegraphics[height=\imageheight,valign=t]{figures/midjourney/25a8c8c9-55c2-48ac-af30-3e1333eb6b76x.jpg}
    &
    % H4
      \vspace{0pt} \includegraphics[height=\imageheight,valign=t]{figures/midjourney/255acf24-263a-4625-93c1-b5757b30e702x.jpg}
    &
    % H5
      \vspace{0pt} \includegraphics[height=\imageheight,valign=t]{figures/midjourney/0f0c96fc-2160-4e59-8331-1bd1bd619ad5x.jpg}
\\
      \textbf{H1:} \prompt{25a8c8c9-55c2-48ac-af30-3e1333eb6b76x.jpg}
    &
      \textbf{H4:} \prompt{255acf24-263a-4625-93c1-b5757b30e702x.jpg}
    & 
      \textbf{H5:} \prompt{0f0c96fc-2160-4e59-8331-1bd1bd619ad5x.jpg}
\\
\end{tabularx}

\noindent
\begin{tabularx}{\textwidth}{
    >{\hsize=.33\hsize}X
    >{\hsize=.33\hsize}X
    >{\hsize=.33\hsize}X
}
    % H6
      \vspace{0pt} \includegraphics[height=\imageheight,valign=t]{figures/midjourney/2be06581-4f12-4b8b-87a4-f77b9e4b375cx.jpg}

    &
    % H8
      \vspace{0pt} \includegraphics[height=\imageheight,valign=t]{figures/midjourney/5f98723a-488e-493e-954b-9cbf38baa69dx.jpg}
    &
    % H10
      \vspace{0pt} \includegraphics[height=\imageheight,valign=t]{figures/midjourney/22a357e6-2425-42b7-8475-dd05c419ecc9x.jpg}
\\
      \textbf{H6:} \prompt{2be06581-4f12-4b8b-87a4-f77b9e4b375cx.jpg}
    &
      \textbf{H8:} \prompt{5f98723a-488e-493e-954b-9cbf38baa69dx.jpg}
    &
      \textbf{H10:} \prompt{22a357e6-2425-42b7-8475-dd05c419ecc9x.jpg}
\\
\end{tabularx}

\noindent
\begin{tabularx}{\textwidth}{X}
    % H3
      \vspace{0pt} \includegraphics[height=\imageheight,valign=t]{figures/midjourney/fb2621f1-b3f0-4cd5-8f93-774836ff1ecex.jpg}
\\
      \textbf{H3:} \prompt{fb2621f1-b3f0-4cd5-8f93-774836ff1ecex.jpg}
\\
\end{tabularx}


\newpage


\noindent
\begin{tabularx}{\textwidth}{
    >{\hsize=.5\hsize}X
    >{\hsize=.5\hsize}X
}
    % H2
      \vspace{0pt} \includegraphics[height=\imageheight,valign=t]{figures/midjourney/a7cbe696-4af4-4af6-9224-c4447c29831cx.jpg}
    &
    % H7
      \vspace{0pt} \includegraphics[height=\imageheight,valign=t]{figures/midjourney/7ca2d0bd-6df7-49c1-91c3-916726216dd8x.jpg}
\\
      \textbf{H2:} \prompt{a7cbe696-4af4-4af6-9224-c4447c29831cx.jpg}
    &
      \textbf{H7:} \prompt{7ca2d0bd-6df7-49c1-91c3-916726216dd8x.jpg}
\\
\end{tabularx}

\noindent
\begin{tabularx}{\textwidth}{XX}
    % H9
      \vspace{0pt} \includegraphics[height=\imageheight,valign=t]{figures/midjourney/896c8280-187b-4b55-a640-9157a9af9a6dx.jpg}
    &

\\
      \textbf{H9:} \prompt{896c8280-187b-4b55-a640-9157a9af9a6dx.jpg}
    &

\\
\end{tabularx}
%TC:endignore



==> TAB/TABLE-HIGH-LARGE.tex <==

%TC:ignore
\noindent
\begin{tabularx}{\textwidth}{
    >{\hsize=.5\hsize}X
    >{\hsize=.5\hsize}X
}
    % H1
      \vspace{0pt} \includegraphics[width=.48\textwidth,valign=t]{figures/midjourney/25a8c8c9-55c2-48ac-af30-3e1333eb6b76x.jpg}
    &
    % H4
      \vspace{0pt} \includegraphics[width=.48\textwidth,valign=t]{figures/midjourney/255acf24-263a-4625-93c1-b5757b30e702x.jpg}
\\
      \textbf{H1:} \prompt{25a8c8c9-55c2-48ac-af30-3e1333eb6b76x.jpg}
    &
      \textbf{H4:} \prompt{255acf24-263a-4625-93c1-b5757b30e702x.jpg}
\\
\end{tabularx}

\noindent
\begin{tabularx}{\textwidth}{
    >{\hsize=.5\hsize}X
    >{\hsize=.5\hsize}X
}
    % H5
      \vspace{0pt} \includegraphics[width=.48\textwidth,valign=t]{figures/midjourney/0f0c96fc-2160-4e59-8331-1bd1bd619ad5x.jpg}
    &
    % H6
      \vspace{0pt} \includegraphics[width=.48\textwidth,valign=t]{figures/midjourney/2be06581-4f12-4b8b-87a4-f77b9e4b375cx.jpg}

\\
      \textbf{H5:} \prompt{0f0c96fc-2160-4e59-8331-1bd1bd619ad5x.jpg}
    &
      \textbf{H6:} \prompt{2be06581-4f12-4b8b-87a4-f77b9e4b375cx.jpg}
\\
\end{tabularx}


      
\noindent
\begin{tabularx}{\textwidth}{
    >{\hsize=.5\hsize}X
    >{\hsize=.5\hsize}X
}
    % H8
      \vspace{0pt} \includegraphics[width=.48\textwidth,valign=t]{figures/midjourney/5f98723a-488e-493e-954b-9cbf38baa69dx.jpg}
    &
    % H10
      \vspace{0pt} \includegraphics[width=.48\textwidth,valign=t]{figures/midjourney/22a357e6-2425-42b7-8475-dd05c419ecc9x.jpg}
\\
      \textbf{H8:} \prompt{5f98723a-488e-493e-954b-9cbf38baa69dx.jpg}
    &
      \textbf{H10:} \prompt{22a357e6-2425-42b7-8475-dd05c419ecc9x.jpg}
\\
\end{tabularx}

\noindent
\begin{tabularx}{\textwidth}{X}
    % H3
      \vspace{0pt} \includegraphics[width=\textwidth,valign=t]{figures/midjourney/fb2621f1-b3f0-4cd5-8f93-774836ff1ecex.jpg}
\\
      \textbf{H3:} \prompt{fb2621f1-b3f0-4cd5-8f93-774836ff1ecex.jpg}
\\
\end{tabularx}


\newpage


\noindent
\begin{tabularx}{\textwidth}{
    >{\hsize=.5\hsize}X
    >{\hsize=.5\hsize}X
}
    % H2
      \vspace{0pt} \includegraphics[height=\imageheight,valign=t]{figures/midjourney/a7cbe696-4af4-4af6-9224-c4447c29831cx.jpg}
    &
    % H7
      \vspace{0pt} \includegraphics[height=\imageheight,valign=t]{figures/midjourney/7ca2d0bd-6df7-49c1-91c3-916726216dd8x.jpg}
\\
      \textbf{H2:} \prompt{a7cbe696-4af4-4af6-9224-c4447c29831cx.jpg}
    &
      \textbf{H7:} \prompt{7ca2d0bd-6df7-49c1-91c3-916726216dd8x.jpg}
\\
\end{tabularx}

\noindent
\begin{tabularx}{\textwidth}{XX}
    % H9
      \vspace{0pt} \includegraphics[height=\imageheight,valign=t]{figures/midjourney/896c8280-187b-4b55-a640-9157a9af9a6dx.jpg}
    &

\\
      \textbf{H9:} \prompt{896c8280-187b-4b55-a640-9157a9af9a6dx.jpg}
    &

\\
\end{tabularx}
%TC:endignore



==> TAB/TABLE-LOW-BAK.tex <==

%TC:ignore
\noindent
\begin{tabularx}{\textwidth}{
    >{\hsize=.33\hsize}X
    >{\hsize=.33\hsize}X
    >{\hsize=.33\hsize}X
}
    % L1
      \vspace{0pt} \includegraphics[height=\imageheight,valign=t]{figures/midjourney/66b13a9f-9c0c-4c9f-aa31-d9c0f2aa8324x.jpg}
    & 
    % L2
      \vspace{0pt} \includegraphics[height=\imageheight,valign=t]{figures/midjourney/6c0066ee-61d7-44a1-bef8-24908db1af47x.jpg}
    & 
    % L3
      \vspace{0pt} \includegraphics[height=\imageheight,valign=t]{figures/midjourney/f41ba10e-05f8-458a-8709-22d1060ea5b2x.jpg}
\\
        \textbf{L1:}
        \prompt{66b13a9f-9c0c-4c9f-aa31-d9c0f2aa8324x.jpg}
    & 
        \textbf{L2:}
        \prompt{6c0066ee-61d7-44a1-bef8-24908db1af47x.jpg}
    & 
        \textbf{L3:}
        \prompt{f41ba10e-05f8-458a-8709-22d1060ea5b2x.jpg}
\\
\end{tabularx}

\noindent
\begin{tabularx}{\textwidth}{
    >{\hsize=.33\hsize}X
    >{\hsize=.33\hsize}X
    >{\hsize=.33\hsize}X
}
    % L4
      \vspace{0pt} \includegraphics[height=\imageheight,valign=t]{figures/midjourney/8d91ae8d-673b-40e0-abed-4ce965353c16x.jpg}
    &
    % L5
      \vspace{0pt} \includegraphics[height=\imageheight,valign=t]{figures/midjourney/71dfc24b-d290-4500-8047-7a0da7bd917bx.jpg}
    &
    % L6
      \vspace{0pt} \includegraphics[height=\imageheight,valign=t]{figures/midjourney/1c67fdcd-b16b-44ba-8f82-16f5f443f7c9x.jpg}
\\
        \textbf{L4:} \prompt{8d91ae8d-673b-40e0-abed-4ce965353c16x.jpg}
    & 
        \textbf{L5:} \prompt{71dfc24b-d290-4500-8047-7a0da7bd917bx.jpg}
    & 
        \textbf{L6:} \prompt{1c67fdcd-b16b-44ba-8f82-16f5f443f7c9x.jpg}
\\
\end{tabularx}

\noindent
\begin{tabularx}{\textwidth}{
    >{\hsize=.33\hsize}X
    >{\hsize=.33\hsize}X
    >{\hsize=.33\hsize}X
}
    % L7
      \vspace{0pt} \includegraphics[height=\imageheight,valign=t]{figures/midjourney/83328d03-585a-4351-b48f-0bfa1cbe72c0x.jpg}
    & 
    % L8
      \vspace{0pt} \includegraphics[height=\imageheight,valign=t]{figures/midjourney/6d8ace44-d363-4654-8e95-0f266bf5886dx.jpg}
    &
    % L9
      \vspace{0pt} \includegraphics[height=\imageheight,valign=t]{figures/midjourney/46ae15d3-20b6-4cf5-914e-db537e760788x.jpg}
\\
        \textbf{L7:} \prompt{83328d03-585a-4351-b48f-0bfa1cbe72c0x.jpg}
    & 
        \textbf{L8:} \prompt{6d8ace44-d363-4654-8e95-0f266bf5886dx.jpg}
    &
        \textbf{L9:} \prompt{46ae15d3-20b6-4cf5-914e-db537e760788x.jpg}
\end{tabularx}

\noindent
\begin{tabularx}{\textwidth}{
    X
}
    % L10
      \vspace{0pt} \includegraphics[height=\imageheight,valign=t]{figures/midjourney/0da6b738-eb79-4b41-b212-2c3a97ada099x.jpg}
\\
        \textbf{L10:}
        \prompt{0da6b738-eb79-4b41-b212-2c3a97ada099x.jpg}
\end{tabularx}
%TC:endignore


==> TAB/TABLE-METRICS-BAK.tex <==
%TC:ignore
\begin{table}[htb]
\small
  \caption{\todo{Comparison of prompts written by workers in Study 3 and Study 4.}}
  \label{tab:promptmeasures}
  \begin{tabular}{lcccclcccccc}
    \toprule
     & \multicolumn{4}{c}{Study 3} & ~ & \multicolumn{4}{c}{Study 4}
     \\
     & \multicolumn{4}{c}{(375 prompts)} & ~ & \multicolumn{4}{c}{\todo{(XXX prompts)}}
     \\
     \cline{2-5} \cline{7-10}
    % \normalsize
    Measure &
    M &
    SD &
    p0 &
    p25 &
    ~ &
    M &
    SD &
    Q0 &
    Q25 & 
    X &
    p
    \\
    \midrule
    % No. of
    Characters
    & 70.77 & 81.26 & 3 & 694 &
    &
    X & X & X & X
    & XX.XX & X.XX
    \\
    % No. of 
    Tokens & 12.54 & 14.65 & 1 & 134 &
    &
    X & X & X & X 
    & X & X.XX
    \\
    % No. of 
    Types & 10.66 & 9.19 & 1 & 60 &
    &
    X & X & X & X
    & X & X.XX
    \\
    TTR & 0.94 & 0.10 & 0.38 & 1 &
    &
    X & X & X & X
    & -- & --
    \\
    % MTLD & 13.70 & 11.72 & 0 & 84 & &
    % xx.xx & xx.xx & xx.xx & xx.xx 
    % \\
    Entropy & 3.73 & 0.48 & 1.5 & 4.36 &
    &
    X & X & X & X 
    & X & X.XX
    \\
    % No. of 
    % Nouns 
    \texttt{NN} & 3.27 & 3.36 & 0 & 33 &
    &
    X & X & X & X
    & X & X.XX
    \\
    % No. of 
    % Adjectives 
    \texttt{JJ} & 1.65 & 1.95 & 0 & 15 &
    &
    X & X & X & X
    & X & X.XX
    \\
    % No. of 
    % Prepositions
    \texttt{IN} & 1.78 & 2.27 & 0 & 21 &
    &
    X & X & X & X
    & X & X.XX
    \\
    % No. of 
    % Verbs 
    \texttt{VB} & 0.36 & 1.02 & 0 & 10 &
    &
    X & X & X & X
    & X & X.XX
    \\
    % No. of 
    % Cardinal numbers
    \texttt{CD} & 0.07 & 0.29 & 0 & 2 &
    &
    X & X & X & X
    & X & X.XX
    \\
% \midrule
%     Mean Levenshtein distance & -- & -- & -- & -- &
%     &
%     28.1 & 22.0 & 0 & 91.3
%     & -- & --
%     \\
%     Word mover distance & -- & -- & -- & -- &
%     &
%     xx.xx & xx.xx & xx.xx & xx.xx 
%     & -- & --
%     \\
  \bottomrule
\end{tabular}
\end{table}
%TC:endignore




==> TAB/TABLE-METRICS-STUDY3-4.tex <==
%TC:ignore
\begin{table}[htb]
\small
  \caption{\todo{Comparison of prompts written by workers in Study 3 and Study 4.}}
  \label{tab:promptmeasures}
  \begin{tabular}{lcccclcccccc}
    \toprule
     & \multicolumn{4}{c}{Study 3} & ~ & \multicolumn{4}{c}{Study 4}
     \\
     & \multicolumn{4}{c}{(375 prompts)} & ~ & \multicolumn{4}{c}{\todo{(XXX prompts)}}
     \\
     \cline{2-5} \cline{7-10}
    % \normalsize
    Measure &
    M &
    SD &
    Min &
    Max &
    ~ &
    M &
    SD &
    Min &
    Max & 
    X &
    p
    \\
    \midrule
    % No. of
    % Characters
    % & 70.77 & 81.26 & 3 & 694 &
    % &
    % X & X & X & X
    % & XX.XX & X.XX
    % \\
    % No. of 
    Tokens & 12.54 & 14.65 & 1 & 134 &
    &
    X & X & X & X 
    & X & X.XX
    \\
    % No. of 
    Types & 10.66 & 9.19 & 1 & 60 &
    &
    X & X & X & X
    & X & X.XX
    \\
    TTR & 0.94 & 0.10 & 0.38 & 1 &
    &
    X & X & X & X
    & -- & --
    \\
    % No. of 
    % Nouns 
    \texttt{NN} & 3.27 & 3.36 & 0 & 33 &
    &
    X & X & X & X
    & X & X.XX
    \\
    % No. of 
    % Adjectives 
    \texttt{JJ} & 1.65 & 1.95 & 0 & 15 &
    &
    X & X & X & X
    & X & X.XX
    \\
    % No. of 
    % Prepositions
    \texttt{IN} & 1.78 & 2.27 & 0 & 21 &
    &
    X & X & X & X
    & X & X.XX
    \\
    % No. of 
    % Verbs 
    \texttt{VB} & 0.36 & 1.02 & 0 & 10 &
    &
    X & X & X & X
    & X & X.XX
    \\
    % No. of 
    % Cardinal numbers
    \texttt{CD} & 0.07 & 0.29 & 0 & 2 &
    &
    X & X & X & X
    & X & X.XX
    \\
% \midrule
%     Mean Levenshtein distance & -- & -- & -- & -- &
%     &
%     28.1 & 22.0 & 0 & 91.3
%     & -- & --
%     \\
%     Word mover distance & -- & -- & -- & -- &
%     &
%     xx.xx & xx.xx & xx.xx & xx.xx 
%     & -- & --
%     \\
  \bottomrule
\end{tabular}
\end{table}
%TC:endignore




==> TAB/TABLE-SETTINGS.tex <==

%TC:ignore
\begin{table}[htb]
\caption{Configuration settings for \todo{Latent Diffusion} used in studies 3 and 4.}
\label{tab:settings}
% \footnotesize
\begin{tabular}{ll}
% \\
\toprule
    Variable  &
	Value
\\
\midrule
	 seed &
     X
\\
	 perceptors &
     ViT-B-16--openai, ViT-B-32--laion2b\_e16
\\
	 latent\_negatives &
     'low quality image'
\\
	 clip\_guidance\_scale
     &
     5000
\\
	 aesthetic\_loss\_scale
	 &
     200
\\
    starting\_timestep
 &
     0.9
\\
    init\_scale
	 &
     1000 
\\
    init\_brightness
	 &
     0.0
\\
    init\_noise
	 &
     0.6
\\
    custom\_schedule\_setting
    &
    [[30, 1000, 8], 'gfpgan:2', [50, 200, 8]]
\\
    opt\_mag\_mul
    &
    10
\\
    opt\_ddim\_eta
    &
    1.4
\\
    opt\_eta\_end
    &
    1
\\
    opt\_temperature
    &
    0.975
\\
\bottomrule
\end{tabular}
\end{table}
%TC:endignore



==> TAB/TABLE-STUDY1-ARTWORKS.tex <==

% \begin{landscape}

%TC:ignore
\begin{table*}[bth]
\caption{\hl{Information on the pilot study's 25~artworks and results obtained from crowd workers on MTurk ($N=30$). As example, Jackson Pollock and his artwork's style was guessed correctly by 90\% and 80\% of the workers, respectively, however none of the workers entered the title of the artwork in any of the task's two input fields.}}
\label{tab:artworks}
% \centering
\footnotesize
\begin{tabularx}{\textwidth}{
    >{\raggedright\arraybackslash}p{2.15cm}
    >{\raggedright\arraybackslash}p{2.8cm}
    >{\raggedright\arraybackslash}X
    l
    l
    l
    l
    l
    l
}
%  & & & \multicolumn{2}{c}{$n=25$}
% \\
\toprule
    \multirow{2}{*}{Artist}  &
% 	\todo{Continent} &
	\multirow{2}{*}{Artwork title}	&
	\multirow{2}{*}{Artistic styles} &
    \multicolumn{2}{l}{\makecell{Artist correct}} &
    \multicolumn{2}{l}{\makecell{Style correct}} &
    \multicolumn{2}{l}{\makecell{Title correct}}
\\
      &
	   &
	   &
    n & \% &
    n & \% &
    n & \%
    \\
\midrule
	 Jackson Pollock &
% 	 N. America &
	 No. 5, 1948 &
	 Abstract expressionism	&
	 27 & 90\% &
  24 & 80\% &
	 0  & 0\%
\\
	 Salvador Dalí &
% 	 Europe &
     The Persistence of Memory &
     Surrealism &
     26 & 86.67\% &
     22 & 73.33\% &
     0 & 0\%
\\
	 Claude Monet  &
% 	 Europe &
	 Impression, Sunrise &
	 Impressionism &
	 25 & 83.33\% &
  22 & 73.33\% &
	 3 & 10\%
\\
     Frida Kahlo &
% 	 N. America &
     Self-portrait with thorn necklace and hummingbird &
     Naïve art, Modern art, Surrealism, Magical Realism, Symbolism, Primitivism, Naturalism, Social realism &
     25 & 83.33\% &
     13 & 52.00\% &
	 7 & 23.33\%
\\
     Pablo Picasso &
% 	 Europe &
     Guernica	&
     Cubism, Surrealism	 	&
     20 & 66.67\% &
     12 & 40.00\% &
     6 & 20.00\% 
\\
	 Grant Wood &
% 	 N. America &
	 American Gothic	&
	 Modernism, Americana Art  &
	 20 & 66.67\% &
  13 & 43.33\% &
	 7 & 23.33\%
\\
     Edvard Munch &
% 	 Europe &
     Anxiety & 	Expressionism, Modern art, Symbolism &
     19 & 63.33\% &
     17 & 56.67\% &
     4 & 13.33\%
\\
     Jeff Koons &
% 	 N. America &
     Balloon Dog &
     Pop art, Contemporary art 	&
     19 & 63.33\% &
     8 & 26.67\% &
     4 & 13.33\%
\\
	 Jasper Johns &
% 	 N. America &
	 Three Flags &
	 Abstract expressionism, Neo-Dada, Modern art, Pop art, Americana Art &
	 18 & 60.00\% &
  10 & 33.33\% &
	 8 & 26.67\%
\\
     Georgia O'Keeffe &
% 	 N. America &
     Jimson Weed 3	 &
     American modernism, Modern art, Modernism, Abstract expressionism, Precisionism  &
     18 & 60.00\% &
     6 & 20\% &
     4	& 13.33\%
\\
     Jean-Michel Basquiat &
% 	 N. America &
     Untitled, 1982 &
     Neo-expressionism, Graffiti, street art &
     16 & 53.33\% &
     19 & 63.33\% &
     2 & 6.67\%
\\
     Piet Mondrian &
% 	 Europe &
     Composition with Red Blue and Yellow & 
     De Stijl, Post-Impressionism, Impressionism, Fauvism, Modern art, Cubism, Expressionism, Abstract art, Modernism &
     15 & 50\% &
     21 & 70\% &
     1	& 3.33\%
\\
	 Mark Rothko &
% 	 N. America &
	 Untitled, 1952	&
	 Abstract expressionism &
	 15 & 50\% &
  18 & 60\% &
     3	& 10.00\%
\\
     Roy Lichtenstein &
% 	 N. America &
     Crying Girl	&
     Pop art  &
     14 & 46.67\% &
     21 & 70\% &
     3	& 10.00\%
\\
	 Edward Hopper &
% 	 N. America &
	 Nighthawks &
	 American realism, Americana Art  &
	 14 & 46.67\% &
  11 & 63.33\% &
	 4	& 13.33\%
\\
	 Paul Klee &
% 	 Europe &
	 Castle and Sun &
	 Expressionism  &
	 13 & 43.33\% &
  12 & 40\% &
     5	& 16.67\%
\\
	 Marc Chagall &
% 	 Other (Belarusian-French)
	 I and the Village &
	 Cubism, Surrealism	&
	 12 & 40\% &
  11 & 36.67\% &
     5	& 16.67\%
\\
 	 Man Ray &
% 	 North America &
 	 Le Violon d'Ingres &
 	 Surrealism, Dada	&
 	 12 & 40\% &
        8 & 26.67\% &
 	 1	& 3.33\%
\\
     Marcel Duchamp &
% 	 Other (French-American) &
     Fountain	&
     Dada	 &
     11 & 36.67\% &
     10 & 33.33\% &
 	 1	& 3.33\%
\\
     Henri Matisse &
% 	 Europe &
     Le bonheur de vivre	&
     Fauvism, Modernism 	&
     11 & 36.67\% &
     8 & 26.67\% &
     2	& 6.67\%
\\
	 Wassily Kandinsky &
% 	 Other (Russian) &
	 Composition VII	&
	 Abstract art  &
	 10 & 33.33\% &
  20 & 66.67\% &
     2	& 6.67\%
\\
	 Joan Miró &
% 	 Europe &
	 The Harlequin's Carnival &
	 Surrealism &
	 10 & 33.33\% &
  13 & 43.33\% &
     2	& 6.67\%
\\
	 Egon Schiele &
% 	 Europe &
	 The Embrace &
	 Expressionism &
	 10 & 33.33\% &
  9 & 30.00\% &
     5	& 16.67\%
\\
     Paul Cézanne &
% 	 Europe &
     The Large Bathers &
     Modern art, Cubism, Post-Impressionism	 &
     9 & 30.00\% &
     17 & 56.67\% &
     0 & 0\%
\\
     Georges Braque &
% 	 Europe &
     Houses at l'Estaque &
     Cubism &
     6 & 20\% &
     13 & 43.33\% &
     2	& 6.67\%
\\
\bottomrule
\end{tabularx}
\end{table*}
%TC:endignore

% \end{landscape}


==> prompts.tex <==
%%% https://tex.stackexchange.com/a/64132/64897
\usepackage{pdftexcmds}

\makeatletter
\newcommand*{\prompt}[1]{%
  \stringcases
    {#1}%
    {%
{1350e6a4-73ab-4cff-860b-933bd0c03ea6x.jpg}{why}%
% {2c9678f5-ab8e-44cb-a02a-a5ca64c63a75x.jpg}{cryptodude wacks cryptobro httpss.mj.runZCpZWs}%
% {4b9f9d94-4d85-4362-be86-a1494ddb06c3x.jpg}{SYMBOL}%
% {5c61fffb-e1a5-40ff-9504-9da8d9a0c956x.jpg}{frog computing on the edge}%
% {61b1bd3c-b74b-46f3-b1a9-6f8f01fabc81x.jpg}{ITS A WAP}%
% {65ed4d7c-e1a4-4cbd-a68c-30d000721e9ax.jpg}{ain't nobody got time for that!}%
% {69a49e79-f406-4920-b980-f08abfc37f77x.jpg}{exodus from heaven matte painting by Michelangelo biblical detailed 8k}%
% {78c0ac28-4e0c-47f1-8117-6d5b4b33f06fx.jpg}{SYMBOL}%
% {8b39cefb-54cf-41a6-a072-5dd09bded1b7x.jpg}{fruits}%
% {dacf6d45-206d-4862-81d8-25b25c2b7ea3x.jpg}{SYMBOL}%
% {e115d414-19f5-41a8-93e9-59775f6fb985x.jpg}{I'm Happy! The happy horse, horse, horse, so full of fun of course, of course!}%
% {e16bd832-0d24-4a8f-becd-db6d53534d5ex.jpg}{how about no}%
% {e3fd984f-bd4f-456c-8ca6-bb4e5f487a82x.jpg}{beach wheres waldo}%
{f41ba10e-05f8-458a-8709-22d1060ea5b2x.jpg}{Asterix at the Robot Games. by Rene Goscinny and Albert Uderzo}%
% {0b704ad8-ce91-4e7b-a67f-cb65990e6918x.jpg}{the art of science httpsstorage.googleapis.comdream-machines-output}%
% {c03400b0-dce1-476a-bf93-d7c216daf8af0x.jpg}{0.jpg}%
% {0c16e567-ae23-48f0-99d1-050f4a3d2fcdx.jpg}{httpss.mj.runr1Xa3M  epophantic mind}%
{0f0c96fc-2160-4e59-8331-1bd1bd619ad5x.jpg}{, ., ., matte painting, 8k cgsociety}%
% {17179b62-55bd-4c94-9a89-5458aa2f646bx.jpg}{second coming rapture of souls}%
% {185ea6ce-bc08-438d-989a-8a81dae774d5x.jpg}{winged demons in hell. by james gurney matte painting fantasy colors CGSociety realistic materials photorealistic postprocessing wow httpst.lylkWt}%
% {21d95935-7271-4421-941a-c59775a0a4e3x.jpg}{scientific artwork}%
{22a357e6-2425-42b7-8475-dd05c419ecc9x.jpg}{portrait of a world war soldier on artstation}%
{25a8c8c9-55c2-48ac-af30-3e1333eb6b76x.jpg}{the foundations of origin, matte painting, genesis, trending on artstation, high resolution}%
% {29d691e4-e7b5-4e8c-acae-890c3c89fcd7x.jpg}{Belgrade Tower post-processing highly detailed matte painting 4k }%
{2be06581-4f12-4b8b-87a4-f77b9e4b375cx.jpg}{The Dude by Glenn Fabry}% OK -- httpss.mj.runPkqzqL  httpss.mj.runQ295nZ 
% {499d4f48-ed9d-4d94-9bb5-74ea9d58dc67x.jpg}{ oil on canvas by James Gurney }%
% {64afcf58-5c72-4579-bdb7-ddce50304787x.jpg}{untitled. oil painting watercolor line drawing by Luke Sywalk James Gurney and Zdzislaw Beksinski}%
% {6befe35d-d4a2-4ab9-8edb-e9425ab946f7x.jpg}{httpss.mj.runTRQGsj  fractures of mind}%
% {6ffd3e50-e10c-4586-b406-601c317e4ea3x.jpg}{seraphim protect the throne of god. by james gurney matte painting fantasy colorful CGSociety realistic materials photo realistic postprocessing amazing httpst.lyFDdV }%
% {54010612-a960-47f5-9865-c432365bc56fx.jpg}{nukes from heaven by Ross Tran Seb McKinnon Hiroshi Yoshida James Gurney highly detailed }%
% {57a2862b-6934-4be5-a103-61df038e0f31x.jpg}{I dont believe in an interventionist god post-processing highly detailed matte painting 4k}%
% {7f66412c-d15e-4728-9703-bfe6fba861d7x.jpg}{quantum atom. science art}%
% {80a0e6d5-517e-4719-b7c9-f64b561612dex.jpg}{avocado beautiful lighting beautiful ambience volumetric lighting global illumination}%
% {825b31a0-de6c-4131-bb39-277bf36728a3x.jpg}{I dont believe in an interventionist god post-processing highly detailed matte painting 4k}%
% {a229a96a-3faf-4bcb-90b4-83241b53d491x.jpg}{When I leave this body I go on what is called through the black hole. Its above the Milky Way galaxy}%
% {a67c90f4-8601-47c2-99a1-135473f3fb86x.jpg}{suit up}%
{a8ad164f-3a2c-4602-af04-0b66ec21d957x.jpg}{httpss.mj.runfAOGx5  I dont believe nicholas cage post-processing highly detailed matte painting 4k }%
% {bde34932-7684-44f2-bd30-d6574c9d89cfx.jpg}{death and destruction becometh }%
% {fdd968b4-cb87-4793-a197-5bd993c2d3efx.jpg}{hole}%
% {d322eebf-d5ae-4968-aaf6-3c314dd011a1x.jpg}{exodus from heaven matte painting by Michelangelo CGSociety detailed 8k}%
% {cf8f6674-3498-490a-a59d-fa06d82233e7x.jpg}{transhuman angel matte painting by Hiroshi Yoshida}%
% {ce109cf5-d0e3-4f52-82e7-18f3cf9513dcx.jpg}{httpss.mj.runElMVUZ  Battal Ebru by Mustafa Duzgunman}%
% {00d75388-a78b-4ce1-b80c-72bc15149a1ax.jpg}{confederation of five thugs}% OK
% {07c42b0b-c3b8-42ff-a5bb-5f047a24e35ex.jpg}{dramatic klaus kinski}% OK
% {08c22f7a-bee6-4cff-aeee-e0fb3ffaefafx.jpg}{Falling Down (1993 ‧ Action/Crime ‧ 1h 53m)}%OK
% {0b7c33e5-f5cb-4aba-87d0-bf0f69bfa21cx.jpg}{indiana jones discovers the lost gold idol, CGSociety, detailed, matte painting, brownleather, indy, postprocessing, 8k}% OK
{0da6b738-eb79-4b41-b212-2c3a97ada099x.jpg}{artwork, academic paper}% OK
% {14550ae4-36e8-456c-8ed0-5cd4ea11cba2x.jpg}{nooooo!!!!11}% OK
% {1566b41c-ec95-40b7-a150-86bb9a7e5cdbx.jpg}{peau salée. YUK!}% OK
% {16528427-5009-4ec4-96c5-4bd64b727e22x.jpg}{oh lord::the creativity}% OK
% {16e1824e-215d-437c-9196-61d511551f6ex.jpg}{put that nozzle down!}% OK
% {1ba3e16a-686e-4608-b856-287d90bb28cax.jpg}{Welcome to the World Institute on World Peace}% OK
{1c67fdcd-b16b-44ba-8f82-16f5f443f7c9x.jpg}{Blind No. 20, Seventeen-foot high Ceiling or Lower, Historical Veridian Green, Indian Yellow Hue, Hansa Yellow Medium (to Mike Kelley)}% OK
% {2d88ddf8-deed-47e6-9871-2ce2879f2f72x.jpg}{indiana jones discovers the lost idol, Hudson River School}% OK
% {3f8e71bf-6a9b-4a97-aff3-87c747bbf912x.jpg}{quantum joy ��}% OK
% {434d7cb3-f0fb-4a5a-8ee4-1514d398751bx.jpg}{indiana jones discovers lost idol, detailed matte painting, brownleather, indy, by Bill Ward}% OK
{46ae15d3-20b6-4cf5-914e-db537e760788x.jpg}{China buys Russia}% OK
% {49957f69-2f8d-46a3-9b4e-552ff462bf39x.jpg}{person, portrait, 180}% OK
% {51916b14-e383-4f11-aaf5-f83191f06753x.jpg}{trololol}% OK
% {51a43477-4325-4145-a3cb-f6500d0d315ax.jpg}{artwork, scientific paper}% OK
{66b13a9f-9c0c-4c9f-aa31-d9c0f2aa8324x.jpg}{Multi-Fidelity MetaLearning for Efficient and Robust AutoDL}% OK
{6c0066ee-61d7-44a1-bef8-24908db1af47x.jpg}{a tweet about bias}% OK
% {6d104b43-e50a-4e7d-9de4-5a68a7381593x.jpg}{hola}% OK
{6d8ace44-d363-4654-8e95-0f266bf5886dx.jpg}{My New Band Is Called Syskill}% OK
% {6efdbda7-a35d-4f72-aa2d-5aaa57277f58x.jpg}{cringeworthy cringy cringe}% OK
{71dfc24b-d290-4500-8047-7a0da7bd917bx.jpg}{Office Space, Bill Lumbergh. ``yeah, we need you to come in on Saturday, mkay?''}% OK !!! https://t.ly/SA6R https://t.ly/U53b https://t.ly/PuQq https://t.ly/u8pC 
% {7d23e1f9-ad67-4660-8d82-f8c83ed12632x.jpg}{indiana jones discovers the lost idol, detailed matte painting, brownleather, indy, by wlop}% OK
% {7e506045-a487-4ea7-9f27-e485cface06dx.jpg}{burning golfball}% OK
{83328d03-585a-4351-b48f-0bfa1cbe72c0x.jpg}{we can do it! propaganda poster}% OK
% {84b26f44-5eaf-4f03-b911-b9bfd0949135x.jpg}{Hand Paintings, cave wall, but in 3D}% OK
% {858c1460-5038-439f-96e0-8c2144ca369cx.jpg}{pink kettlebell}% OK
{8d91ae8d-673b-40e0-abed-4ce965353c16x.jpg}{amazing green screen effect}% OK
% {958300e0-ce28-4531-9ed5-30864f706941x.jpg}{indiana jones discovers the lost idol, CGSociety, detailed, matte painting, brownleather, indy, postprocessing, 8k}% OK
% {9b36ab76-3ddc-4e46-bbc9-8f7358425eebx.jpg}{quantum joy}% OK
% {a8726d95-ddab-437f-97c2-483d339fa2f8x.jpg}{pi accelerator}% OK
% {aadd8072-351b-4942-b5e2-9af803faac5bx.jpg}{factoid. by Mark Bradford}% OK
% {ad5652c9-3dc3-4ec0-92a5-92a6d7b3ace9x.jpg}{proud producer of spaghetti code}% OK
% {b13dc8e8-1181-41c5-9cc2-7585c1977657x.jpg}{run to the hills}% OK
% {b3274a74-d445-41af-a6b0-c5b566b3fa7dx.jpg}{klaus kinski}% OK
% {b9dd4cfa-a88c-4b16-948d-fd6f7a506d2fx.jpg}{When you're gone, how can I even try to go on?}% OK
% {bb87a699-5d28-4310-ac57-7107a8368a51.jpg}{indiana jones discovers lost idol, detailed matte painting, brownleather, indy, by Joseph Cross}% OK
% {c074b1a0-0de6-4456-9449-5e6f6ba9d186 1250x.jpg}{12:50, press Return}% OK
% {c24197d6-d495-453a-aae7-c8cb7cee5165x.jpg}{graffiti of a graffiti}% OK
% {c3ec8059-0b80-4d99-8b04-08cc3508d79dx.jpg}{the wardrobe of sound. Feel the beat.}% OK
% {d01e3bab-3135-4dfa-8e7d-31e0956963bbx.jpg}{pump action coca cola bottle}% OK
% {d6b1715f-edcf-4226-9806-b5e5fecd831bx.jpg}{woman gives birth in metro station. emergency birth. photograph, Pulitzer Prize}% OK
{ea074a0c-6c40-462e-9e25-019219f6c270x.jpg}{Cueva}% OK
{fb2621f1-b3f0-4cd5-8f93-774836ff1ecex.jpg}{buck, Hudson River School}% OK
% {177d4ac4-86a3-4cce-a580-35a303399ba9x.jpg}{rage, by Jackson Pollock}% OK
% {2281e74c-6fc3-4669-8b2a-a866e0c6437dx.jpg}{primal scream, poster art}% OK
{255acf24-263a-4625-93c1-b5757b30e702x.jpg}{eclectic interior of the mind}% OK
% {337a656e-2862-4cfb-a9c0-f0eb3fddddbcx.jpg}{eclectic mind, eclectic soul}% OK
% {345b1c0f-fe91-42f4-9e62-191c9714e152x.jpg}{goddess of plumage}% OK
% {3ff2c24c-6786-4bff-992f-bbe613137e4cx.jpg}{repent, sinners! painting, by Mark Bradford}% OK
% {454567a1-0a1a-470b-be68-d5097a086a98x.jpg}{family, children's drawing}% OK
% {5562fa48-a0f9-42c4-aa05-53f5d195bb3dx.jpg}{antagonist. by Luke Sywalk and Beksinski}% OK
% {58355346-82a4-450f-a813-9beb224e47a8x.jpg}{shine on you shiny demon}% OK
{5f98723a-488e-493e-954b-9cbf38baa69dx.jpg}{a moment of silence for our fallen heroes. War memorial. central. CGSociety, painting, postprocessing}% OK
% {76203c33-4049-481f-a471-0145a6acbafex.jpg}{harbinger of light darkness shall forever cede to the light}% OK
{7ca2d0bd-6df7-49c1-91c3-916726216dd8x.jpg}{fantastic wardrobe of the inner sanctuary comes to life in giant birtation of the soul}% OK
% {7e7e9e56-2912-4b27-afe7-461adde7fcaax.jpg}{interior melting with time and space like eternity facing the mindful evidence of its existence}% OK
% {84fc1ddf-8dd2-4ef8-ba0b-9fc4dbbdb81ex.jpg}{beacon of light in the darkness}% OK
% {851258aa-9064-4870-af22-b1c9068c9ac1x.jpg}{people bow to the demon. matte painting, detailed}% OK
{896c8280-187b-4b55-a640-9157a9af9a6dx.jpg}{tidal wave, matte painting, rendered in octane, ghibli, 8k \#epic \#wow trending on wikiart}% OK
% {9d526b6b-df89-4186-8746-5eeb31b29d83x.jpg}{Urania cover}% OK
{a7cbe696-4af4-4af6-9224-c4447c29831cx.jpg}{vikings. by Dan Mumford, matte painting, Studio Ghibli}% OK
% {ceb722b6-7ea6-4f72-921b-3a03271470e4x.jpg}{fantastic journey. by Beksinski and T. Burgler }% OK
% {d226904c-0704-4a4a-8c38-9502a1005cf5x.jpg}{attack of the monster Cthulhu. matte painting, detailed, photorealistic}% OK
% {d7de3147-ca5f-4180-91a4-a4e5f9355749x.jpg}{the end of the World. by james gurney matte painting, CGSociety, fantasy, full of colors, wow, ultra photorealistic, wow, postprocessing}% OK
% {dde361ad-fc27-41a7-9d14-74ec9bed3d16x.jpg}{Spiral. Album Cover. by Nine Inch Nails% OK
% {eb61fb33-3e2f-4a73-ac13-f2f99f4aca46x.jpg}{machine of loving grace}% OK
% {ee9d9722-d285-48d0-8a34-c48242fa1d33x.jpg}{swept away with the tide. oil on canvas, ultra photorealistic, detailed, matte painting, fantastic, wow}% OK
    }%
    {n/a}%
}%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\stringcases}[3]{%
  \romannumeral
    \str@case{#1}#2{#1}{#3}\q@stop
}
\newcommand{\str@case}[3]{%
  \ifnum\pdf@strcmp{\unexpanded{#1}}{\unexpanded{#2}}=\z@
    \expandafter\@firstoftwo
  \else
    \expandafter\@secondoftwo
  \fi
    {\str@case@end{#3}}
    {\str@case{#1}}%
}
\newcommand{\str@case@end}{}
\long\def\str@case@end#1#2\q@stop{\z@#1}
\makeatother



